An accurate and flexible analog emulation of AdEx neuron dynamics in silicon

Analog neuromorphic hardware promises fast brain emulation on the one hand and an efficient implementation of novel, brain-inspired computing paradigms on the other. Bridging this spectrum requires flexibly configurable circuits with reliable and reproducible dynamics fostered by an accurate implementation of the targeted neuron and synapse models. This manuscript presents the analog neuron circuits of the mixed-signal accelerated neuromorphic system BrainScaleS-2. They are capable of flexibly and accurately emulating the adaptive exponential leaky integrate-and-fire model equations in combination with both current- and conductance-based synapses, as demonstrated by precisely replicating a wide range of complex neuronal dynamics and firing patterns.

==> preamble/circuits.tex <==
\makeatletter

\ctikzset{tripoles/double gm amp/output height/.initial=0.3} 

\pgfdeclareshape{double gm amp}
{
    \savedmacro{\ctikzclass}{\edef\ctikzclass{amplifiers}}
    \saveddimen{\scaledRlen}{\pgfmathsetlength{\pgf@x}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}}
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/gm amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/gm amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \ctikzvalof{tripoles/op amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/gm amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/gm amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/gm amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/gm amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/gm amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/gm amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
        \savedanchor\up{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@y=\ctikzvalof{tripoles/gm amp/height}\pgf@circ@scaled@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/gm amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \ctikzvalof{tripoles/gm amp/up pos}}{
            \pgfpoint{
            \ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/gm amp/height 2}\pgf@circ@res@up}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    \anchor{out1}{
        \northwest
        \pgf@y=\ctikzvalof{tripoles/double gm amp/output height}\pgf@y
        \pgf@x=-\pgf@x
    }
    \anchor{out2}{
        \northwest
        \pgf@y=\ctikzvalof{tripoles/double gm amp/output height}\pgf@y
        \pgf@y=-\pgf@y
        \pgf@x=-\pgf@x
    }
    %
    \savedanchor\leftedge{%
        \pgfmathsetlength{\pgf@circ@scaled@Rlen}{\ctikzvalof{\ctikzclass/scale}\pgf@circ@Rlen}
        \pgf@x=-\ctikzvalof{tripoles/gm amp/width}\pgf@circ@scaled@Rlen
        \pgf@x=.5\pgf@x
        \pgf@x = \ctikzvalof{tripoles/gm amp/port width}\pgf@x
        \pgf@y=0pt
    }
    \anchor{leftedge}{\leftedge}
    \anchor{rightedge}{\leftedge \pgf@x =-\pgf@x }
    \anchor{bin up}{
        \inOneFixed
        \pgf@ya=\pgf@y \leftedge \pgf@y=\pgf@ya
    }
    \anchor{bin down}{
        \inOneFixed
        \pgf@y=-\pgf@y
        \pgf@ya=\pgf@y \leftedge \pgf@y=\pgf@ya
    }
    \anchor{b-}{
        \inOne
        \pgf@ya=\pgf@y \leftedge \pgf@y=\pgf@ya
    }
    \anchor{b+}{
        \inOne
        \pgf@y=-\pgf@y
        \pgf@ya=\pgf@y \leftedge \pgf@y=\pgf@ya
    }
    \anchor{bout}{
        \leftedge
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    %
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

    \anchor{text}{
        \ifpgf@circ@center@text
            \pgf@x=\dimexpr -.6\wd\pgfnodeparttextbox\relax
        \else
            \leftedge
            \pgfmathsetlength{\pgf@x}{\pgf@x + \ctikzvalof{left text distance}}
        \fi
        \pgf@y=\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
    }
    \backgroundpath{
        \pgfsetcolor{\ctikzvalof{color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@scaled@Rlen=\scaledRlen

        \pgfscope
            \newdimen\pgf@circ@res@right@double
						\pgf@circ@res@right@double=2\pgf@circ@res@right

            \pgf@circ@setlinewidth{tripoles}{\pgflinewidth}
            \pgftransformxshift{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@step
            %
            \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right@double}{0}} %
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/gm amp/height 2}\pgf@circ@res@up}}%
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}} %
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}} %
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right@double}{\ctikzvalof{tripoles/gm amp/height 2}\pgf@circ@res@down}}%
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/gm amp/font} \ifpgf@circuit@oa@iplusup\pgf@circ@ampli@plus\else\pgf@circ@ampli@minus\fi}


        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/gm amp/input height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/gm amp/font} \ifpgf@circuit@oa@iplusup\pgf@circ@ampli@minus\else\pgf@circ@ampli@plus\fi}


	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\ctikzvalof{tripoles/double gm amp/output height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/double gm amp/output height}\pgf@circ@res@up}} %

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\ctikzvalof{tripoles/double gm amp/output height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/gm amp/port width}\pgf@circ@res@right}{\ctikzvalof{tripoles/double gm amp/output height}\pgf@circ@res@down}} %
        \pgfsetrectcap
        \pgfusepath{draw}

    }
}

\long\def\pgfaddtoshape#1#2{%
  \begingroup
  \def\pgf@sm@shape@name{#1}%
  \let\anchor\pgf@sh@anchor
  \let\backgroundpath=\pgf@sh@bgpath
  \let\beforebackgroundpath=\pgf@sh@beforebgpath
  #2%
  \endgroup
}
 
\newif\ifthox
\pgfkeys{/tikz/circuitikz/tripoles/nmos/thox/.is if=thox}
\pgfkeys{/tikz/circuitikz/tripoles/pmos/thox/.is if=thox}

\pgfaddtoshape{nmos}{
	\beforebackgroundpath{%
	\ifthox
        \pgfsetcolor{\ctikzvalof{color}}%
%
        \pgfscope%
		\pgfpathmoveto{
			\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@up}
			}
		\pgfpathlineto{\pgfpointadd{
			\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@up}
			}{\pgfpoint{2pt}{0pt}}
			}
		\pgfpathlineto{\pgfpointadd{
			\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}
			}{\pgfpoint{2pt}{0pt}}
			}
		\pgfpathlineto{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}}

            %
            %
            \pgfpathclose%
        \endpgfscope%
        \pgfsetrectcap%
	\pgfsetlinewidth{2\pgflinewidth}
        \pgfusepath{draw}%
	\else
	\fi
	}%
}

\pgfaddtoshape{pmos}{
	\beforebackgroundpath{%
	\ifthox
        \pgfsetcolor{\ctikzvalof{color}}%
%
        \pgfscope%
		\pgfpathmoveto{
			\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}
			}
		\pgfpathlineto{\pgfpointadd{
			\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}
			}{\pgfpoint{2pt}{0pt}}
			}
		\pgfpathlineto{\pgfpointadd{
			\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@down}
			}{\pgfpoint{2pt}{0pt}}
			}
		\pgfpathlineto{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@down}}

            %
            %
            \pgfpathclose%
        \endpgfscope%
        \pgfsetrectcap%
	\pgfsetlinewidth{2\pgflinewidth}
        \pgfusepath{draw}%
	\else
	\fi
	}%
}

\tikzset{
	thox/.style = {
		/tikz/circuitikz/tripoles/nmos/gate width=0.67,
		/tikz/circuitikz/tripoles/pmos/gate width=0.67,
		/tikz/circuitikz/tripoles/nmos/thox,
		/tikz/circuitikz/tripoles/pmos/thox
		}
	}

\makeatother


==> preamble/panels.tex <==
\newcounter{panel}
\newcounter{npanels}

\makeatletter
\newcommand{\labeltext}[3][]{%
	\@bsphack%
	\csname phantomsection\endcsname%
	\def\tst{#1}%
	\def\labelmarkup{\emph}%
	%
	\def\refmarkup{}%
	\ifx\tst\empty\def\@currentlabel{\refmarkup{#2}}{\label{#3}}%
	\else\def\@currentlabel{\refmarkup{#1}}{\label{#3}}\fi%
	\@esphack%
	\labelmarkup{#2}%
	}
\newcommand{\panelcaption}[1]{%
	\ifnum\value{panel}=0{\gdef\panelcaptions{}}\else{}\fi
	\addtocounter{figure}{1}%
	\refstepcounter{panel}%
	\csname phantomsection\endcsname%
	\def\subcaptionlabel{#1}%
	\edef\@currentlabel{\thefigure\,\Alph{panel}}%


  \cref@constructprefix{figurepanel}{\cref@result}%
  \protected@edef\@currentlabelname{\thefigure\,\Alph{panel}}%
  \protected@edef\cref@currentlabel{%
    [figurepanel][][\cref@result]%
    \thefigure\,\Alph{panel}%
  }


	\ifx\subcaptionlabel\empty{}\else\protected@xdef\panelcaptions{\panelcaptions \textbf{(\Alph{panel})}~#1 }\fi
	\addtocounter{figure}{-1}
	}
\makeatother

\let\oldfigure\figure
\let\oldendfigure\endfigure
\def\figure{\setcounter{npanels}{\value{figure}}\oldfigure}
\def\endfigure{%
	\ifnum\value{panel}>0{\ifnum\value{npanels}=\value{figure}{\addtocounter{figure}{1}}\else{}\fi}\else{}\fi
	\oldendfigure
	\setcounter{panel}{0}}

\newenvironment{panels}{\begin{tikzpicture}}{\end{tikzpicture}}

	\usepackage{xparse}
	\NewDocumentCommand\panel{ O{} d() u{at} r() m m m }{%
		\node[inner sep=0pt,#1] (#2) at (#4) {\panelcaption{#6}\label{#7}};
		\node[inner sep=0pt,#1] (#2) at (#4) {#5};
		}
	\NewDocumentCommand\panellabel{ O{} d() u{at} r() m }{\node[anchor=north west,#1] at (#4) {#5};}

\tikzset{
	panel/.style={inner sep=0pt,
		execute at begin node={\tikzset{anchor=center, inner sep=.33333em}}},
		%
	label/.style={anchor=north west,font=\bfseries,outer sep=0pt,inner sep=0pt},
	caption/.style={
		append after command={\pgfextra \node[inner sep=0pt]
		at (\tikzlastnode) {\panelcaption{#1}\label{\panellabelhandle}};
		\endpgfextra
		}},
	handle/.code={
		\gdef\panellabelhandle{#1}
	},
	%
	marker/.style args = {#1:#2}{
		append after command={\pgfextra \node[anchor=#2]
		at (\tikzlastnode.north west) {#1};
		\endpgfextra
	    }
	    },
	marker/.default={:north east}
	}



==> preamble/wisker.tex <==
 \makeatletter
 \pgfkeys{/tikz/wisker length/.initial = 1.2cm}
 \pgfkeys{/tikz/wisker width/.initial = 1.2cm}
 \pgfkeys{/tikz/wisker outline/.initial = 0.8pt}
 \newif\ifmirrorshape
 \pgfkeys{/tikz/mirror/.is if=mirrorshape}


 \pgfdeclareshape{wisker}
 {
	 \savedanchor\centerpoint{
		 \pgf@x = .5\wd\pgfnodeparttextbox
		 \pgf@y = .5\ht\pgfnodeparttextbox
	 }
	 \anchor{center}{\centerpoint}
	 \saveddimen\tunersize{\pgf@x=\pgfkeysvalueof{/tikz/wisker length}}

	 \savedanchor\wiskerpoint{
		 \ifmirrorshape
			 \pgf@x=+\pgfkeysvalueof{/tikz/wisker length}
		 \else
			 \pgf@x=-\pgfkeysvalueof{/tikz/wisker length}
		 \fi
		 \pgf@x=.35\pgf@x
		 \pgf@y=-\pgfkeysvalueof{/tikz/wisker length}
		 \pgf@y=.35\pgf@y
	 }
	 \anchor{handle}{\wiskerpoint}


	 \backgroundpath{
		 \pgfsetarrows{-stealth}
		
		 \ifmirrorshape
			 \pgfsetstrokecolor{white}
			 \pgfsetlinewidth{\pgfkeysvalueof{/tikz/wisker width}+\pgfkeysvalueof{/tikz/wisker outline}}
			 \pgfpathmoveto{\pgfpointadd{\pgfpointscale{0.35}{\pgfpoint{\tunersize}{-\tunersize}}}{\pgfpoint{0.7*\pgfkeysvalueof{/tikz/wisker outline}}{-0.7*\pgfkeysvalueof{/tikz/wisker outline}}}}
			 \pgfpathlineto{\pgfpointadd{\pgfpointscale{0.35}{\pgfpoint{-\tunersize}{\tunersize}}}{\pgfpoint{-2*0.7*\pgfkeysvalueof{/tikz/wisker outline}}{2*0.7*\pgfkeysvalueof{/tikz/wisker outline}}}}
			 \pgfusepath{stroke}
			 
			 \pgfsetstrokecolor{black}
			 \pgfsetlinewidth{\pgfkeysvalueof{/tikz/wisker width}}
			 \pgfpathmoveto{\pgfpointscale{0.35}{\pgfpoint{\tunersize}{-\tunersize}}}
			 \pgfpathlineto{\pgfpointscale{0.35}{\pgfpoint{-\tunersize}{\tunersize}}}
			 \pgfusepath{stroke}
		\else
			 \pgfsetstrokecolor{white}
			 \pgfsetlinewidth{\pgfkeysvalueof{/tikz/wisker width}+\pgfkeysvalueof{/tikz/wisker outline}}
			 \pgfpathmoveto{\pgfpointadd{\pgfpointscale{0.35}{\pgfpoint{-\tunersize}{-\tunersize}}}{\pgfpoint{-0.7*\pgfkeysvalueof{/tikz/wisker outline}}{-0.7*\pgfkeysvalueof{/tikz/wisker outline}}}}
			 \pgfpathlineto{\pgfpointadd{\pgfpointscale{0.35}{\pgfpoint{\tunersize}{\tunersize}}}{\pgfpoint{2*0.7*\pgfkeysvalueof{/tikz/wisker outline}}{2*0.7*\pgfkeysvalueof{/tikz/wisker outline}}}}
			 \pgfusepath{stroke}
			 
			 \pgfsetstrokecolor{black}
			 \pgfsetlinewidth{\pgfkeysvalueof{/tikz/wisker width}}
			 \pgfpathmoveto{\pgfpointscale{0.35}{\pgfpoint{-\tunersize}{-\tunersize}}}
			 \pgfpathlineto{\pgfpointscale{0.35}{\pgfpoint{\tunersize}{\tunersize}}}
			 \pgfusepath{stroke}
		\fi
		 %
		 %
		 %
	 }
 }

 \makeatother

